Federated Data Science to Break Down Silos [Vision]

Similar to Open Data initiatives, data science as a community has launched initiatives for sharing not only data but entire pipelines, derivatives, artifacts, etc. (Open Data Science). However, the few efforts that exist focus on the technical part on how to facilitate sharing, conversion, etc. This vision paper goes a step further and proposes KEK, an open federated data science platform that does not only allow for sharing data science pipelines and their (meta)data but also provides methods for efficient search and, in the ideal case, even allows for combining and defining pipelines across platforms in a federated manner. In doing so, KEK addresses the so far neglected challenge of actually finding artifacts that are semantically related and that can be combined to achieve a certain goal.

==> sections/intro-backup.tex <==
%!TEX root = ../paper.tex

\section{Introduction}
\label{sec:introduction}

Open Data initiatives have led to the development of Open Data portals that provide machine-readable and structured datasets in topics, such as health, education,  transportation, agriculture, and food. They are driven, for example, by governments, e.g., \href{https://www.data.gov/}{\underline{USA}}, \href{https://open.canada.ca/en}{\underline{Canada}}, \href{https://data.europa.eu/euodp}{\underline{EU}}, \href{https://data.ny.gov/browse}{\underline{New York}}, \href{https://www.donneesquebec.ca/}{\underline{Quebec}},  or organizations, such as \href{https://www.who.int/data/gho}{\underline{WHO}} and \href{https://data.wto.org/}{\underline{WTO}}, and provide access to thousands of datasets. 
Encouraged by the availability of this data and the FAIR principles~\cite{wilkinson2016fair}, data science projects are increasingly striving at making datasets and related data science experimentation automatically and efficiently findable, accessible, interoperable, and reusable. This includes sharing data science pipelines and derived insights, such as code, notebooks, technical papers as well as other (non-standardized) artifacts describing the rationale for the experimentation. 

%Open data initiatives have led to the development of Open Data portals that provide machine-readable and structured datasets in topics, such as health, education, social policies, transportation, agriculture, and food. These open data portals are established at different granularities. Countries, such as the \href{https://www.data.gov/}{\underline{USA}} and \href{https://open.canada.ca/en}{\underline{Canada}}, have open data portals with more than 224K and 83K datasets, respectively. A state like \href{https://data.ny.gov/browse}{\underline{New York}} has a data portal with about 5K datasets while the data portal of a province like \href{https://www.donneesquebec.ca/}{\underline{Quebec}} has more than 1200 datasets. The open data portals of the World Health Organization (\href{https://www.who.int/data/gho}{\underline{WHO}}) and Trade Organization (\href{https://data.wto.org/}{\underline{WTO}}) have thousands of datasets in health and economy. %The European Union open data portal~\cite{EU} offers more than 15K datasets. 

%A growing number of data science projects use such open data to underpin the process of decision making and policy making via data science experimentation, i.e., pipelines and derived insights. Such data science experimentation begins with the process of integrating and pre-processing multiple datasets but also includes code, notebooks, technical papers as well as other (non-standardized) artifacts describing the rationale for the experimentation. 
%ncouraged by the scientific community and reproducibility efforts, the vision of the FAIR principles~\cite{wilkinson2016fair} for data science has been moved forward striving for datasets and related data science experimentation becoming automatically and efficiently findable, accessible, interoperable, and reusable.

Unfortunately, despite artifacts of experimentation and creation of pipelines becoming increasingly more open, most of the artifacts %associated with derivation and sharing of insights and data science models 
are scattered across various open source repositories, such as GitHub or GitLab. Furthermore, documentation describing the work is available along with code on Jupyter notebooks, blogs in domains, such as Medium, and open repositories of preprints, e.g., ArXiv. 
Recently, we have therefore seen the rise of initiatives and projects, such as Agora~\cite{Agora}, with the goal of providing the foundations of how to technically combine data science pipelines in decentralized and dynamic environments, where data, algorithms, etc. are distributed.
While these projects concentrate on the question \emph{how to technically combine artifacts}, they neglect questions, such as \emph{what artifacts should be combined (across platforms, servers, etc.) to achieve a certain goal} and \emph{how do we find artifacts that are semantically similar or connected}. 
In this vision paper, we are closing this gap by proposing a federated data science platform, called {\FDSP}~\footnote{\hitext{KEK is the initials of the authors' first name. Kek means "raiser up of the light" in ancient Egypt.}}, that addresses these neglected questions to break down silos in data science (DS). 

Achieving this vision begins with the need to find, combine, and reuse artifacts as they are currently locked away in silos. There is no well-defined way of sharing these artifacts enhanced with semantic descriptions or even general metadata, neither much within a given data science platform and definitely not across multiple platforms. Thus, data scientists cannot automatically find relevant datasets and build a new pipeline on top of related ones since there is no way to identify them. 
As a practical use case and example, let us consider the case of reproducing experimental results of published articles, and analyzing insights driven from datasets.  

\begin{figure*}
\ncp\ncp\ncp\ncp\ncp
  \centering
  \includegraphics[width=0.79\linewidth]{figures/KEKRunningExample.pdf}
  \ncp\ncp\ncp\ncp\ncp
  \caption{An overview of data science (DS) experimentations suffering from silos of data, pipelines, and insights. These silos prevent communication among the DS community 
  %to find answers to their questions 
  and lead to consuming more time in data preparation, authoring pipelines, and finding insights related to datasets. The required automation to break down silos is denoted in red color.
  %The dotted red lines and squares denote different aspects demanding automation to break down silos in data science.
}   
  \label{fig:silos}
  \ncp\ncp\ncp\ncp
\end{figure*}

\textbf{Example. } The problem is illustrated %with an example scenario 
in Figure~\ref{fig:silos} -- Laboratory 1 has a pipeline in a Java-based machine learning library (MLLib) operating on Dataset 1 to produce insights after enriching Dataset 1 with a local dataset; while Laboratory 2 has a pipeline in a Python machine learning library (Sklearn) that operates on Dataset 2 to produce insights described in a recent paper. At a \emph{semantic} level, Dataset 2 could be joined with Datasets 1 and 3. Similarly, at a \emph{semantic} level, the pipelines are equivalent; albeit in different programming languages and libraries. Yet, currently neither laboratory has any way to understand exactly what has been accomplished in the scientific community with respect to the datasets available at a specific data portal, e.g., Data Portal 1.

Existing data science platforms, such as 
\href{https://mlflow.org/}{\underline{MLFlow}}
and 
\href{https://www.blog.google/products/google-cloud/cloud-automl-making-ai-accessible-every-business/}{\underline{AutoML}}, tend to expand silos by locking-in pipelines and driven insights with limited or no collaboration support to force scientists to use the same platform. While a number of data science portals already exist, such as
\href{https://www.openml.org/}{\underline{OpenML}} and
\href{https://www.kaggle.com/}{\underline{Kaggle}}, they still expect each user to load all open datasets, pipelines, and insights into their specific platforms -- even before users can collaborate. 
% And even though they are quite helpful, the use of any single central platform represents another silo. Although scientists prefer to easily move between platforms based on who they collaborate with and how much they want to share, this is not really supported by existing portals and platforms. 
In general, access to this community effort should not be restricted to a limited set of APIs, as in Kaggle. %Instead, 
A more flexible mechanism to allow sharing of \textbf{datasets} and their associated \textbf{data science} artifacts is needed.

% Kaggle~\footnote{\url{https://www.kaggle.com/}}

%In this paper we therefore propose a federated data science platform, called {\FDSP}.%\footnote{KEK is the initials of the authors' first name. Kek means "raiser up of the light" in ancient Egypt.} 
%to break down silos in data science (DS). 
{\FDSP} therefore aims to provide a mechanism for the scientific community to discover and learn from each other's work automatically. 
In particular, {\FDSP} will help (i) discover and extract relevant data, (ii) enable scientists to collaborate more effectively regardless of the DS platforms they use, (iii) support efficient discovery of the most recent insights related to a dataset, (iv) enable scientists to reuse and combine (parts of) existing DS pipelines in novel ways, (v) enable reproducibility of experimental results with ease, and (vi) encourage innovative applications to automate several aspects of DS based on the most recent DS experimentation.

One of the key concepts to enable this vision and overcome silos is to abstract from syntactical differences of existing platforms and instead focus on the semantics of datasets, artifacts, and pipelines. Once we understand the semantics, we can more easily identify similar or matching artifacts and combine them %using wrappers or similar technologies to combine them 
in a federated manner. 
Instead of creating yet another silo by limiting {\FDSP} to a non-flexible standard, another key consideration is to retain a maximal degree of flexibility by capturing metadata and semantics in a flexible graph format.
In our example from Figure~\ref{fig:silos}, for instance, each laboratory's artifacts (stored in databases, file systems, or from a GitHub repository) are represented and indexed by an abstract graph representation that can be shared with other laboratories as illustrated in Figure~\ref{fig:overview}. 
%disentangle the platform specific configurations from the semantics of 
\hitext{By using an abstract representation of the semantics of operations in pipelines, {\FDSP} enables identifying semantically similar pipelines across platforms. TODO: back up with example high-level operations!!!
}

\hitext{
Another key concept to avoid locking users into yet another platform is that {\FDSP} is envisioned as a federated platform of independent {\FDSP} instances so that these instances can collaborate without having to rely on a central instance or authority.  
Consider, for example, a new dataset becoming available at a particular instance; using the {\FDSP} infrastructure we first extract characteristics from the new dataset, capture provenance, etc. in a labeled graph (part of {\FDSP}'s DSKG) covering characteristics as well as which processes, pipelines, and other datasets were involved in creating this dataset. 
Since these artifacts can reside on other {\FDSP} instances, we obtain links to partial graphs at other instances. 
Apart from enabling classic search-engine-style dataset or artifact search~\cite{ChapmanSKKIKG20} and federated query processing over distributed knowledge graphs~\cite{FedX} to compute graph queries over DSKGs, we can use {\FDSP}'s infrastructure, for instance, to extract and learn features and train ML models to propose compatible (non-local) pipelines that have been applied to similar (non-local) datasets.
}

The remainder of this paper is organized as follows. Section~\ref{sec:platform} presents an architectural overview of {\FDSP}. 
% and discusses how {\FDSP} could be used in practice. 
In Section~\ref{sec:opp}, we discuss the research gaps for reaching our vision. Section~\ref{sec:rw} puts our vision into context with related proposals and the state of the art and Section~\ref{sec:con} concludes the paper.











